Optimal security hardening over a probabilistic attack graph: a case study of an industrial control system using the CySecTool tool

CySecTool is a tool that finds a cost-optimal security controls portfolio in a given budget for a probabilistic attack graph. A portfolio is a set of counter-measures, or controls, against vulnerabilities adopted for a computer system, while an attack graph is a type of a threat scenario model. In an attack graph, nodes are privilege states of the attacker, edges are vulnerabilities escalating privileges, and controls reduce the probabilities of some vulnerabilities being exploited. The tool builds on an optimisation algorithm published by Khouzani et al. (2019), enabling a user to quickly create, edit, and incrementally improve models, analyse results for given portfolios and display the best solutions for all possible budgets in the form of a Pareto frontier. A case study was performed utilising a system graph and suspected attack paths prepared by industrial security engineers based on an industrial source with which they work. The goal of the case study is to model a supervisory control and data acquisition (SCADA) industrial system which, due to having the potential to harm people, necessitates strong protection while not allowing the use of typical penetration tools like vulnerability scanners. Results are analysed to show how a cyber-security analyst would use CySecTool to store cyber-security intelligence and draw further conclusions.

==> tables/costs.tex <==
\renewcommand\tabularxcolumn[1]{m{#1}}% for vertical centering text in X column

\begin{landscape}
	\begin{xltabular}{\columnwidth}{XXX}
		\caption{Mitigations expressed in basic actions as defined in \autoref{tab:actions}.}
		\label{tab:mitigations_costs} \\
		\toprule
		Control                                                            & Actions                                                                                                                                                          & Rationale                                                                                                                                                                                                                        \\*
		\endfirsthead
		\toprule
		Control                                                            & Actions                                                                                                                                                          & Rationale                                                                                                                                                                                                                        \\*
		%
		\endhead
		%
		\endfoot
		%
		\endlastfoot
		%
		\hline
		ViewX and OT Active Directory   removed from IT zone.              & 3x Extra employee. \newline 3x Taking away permissions. \newline 1x New ICS software feature. \newline 1x New PC software. & Establishing admin team at the   OT.\newline ViewX reprogrammed to use the   new AD instance.\newline New AD instance.                                                                   \\
		\hline
		Access to OT from IT limited to   WebX.                            & 2x Above                                                                                                                                                         & Establishing incident response   team at the OT.                                                                                                                                                                                 \\
		\hline
		Firewall, antivirus and patch   manager installed on thin clients. & 1x Extra employee.\newline 3x New PC software.                                                                           & Extra administrator to take   care of the policy.\newline Antivirus and firewall software.                                                                                               \\
		\hline
		Company issued and periodically   formatted drives only.           & 10x Buying a tool.                                                                                                                                               & We need to buy enough pen   drives for all the employees and keep them from using their own.                                                                                                                                     \\
		\hline
		Single-use CDs only recorded   directly by SCADA software.         & Above +\newline 1x New ICS software feature.\newline 2x Taking away perms                                                & The system needs to be adapted   to burn CDs.\newline Using CDs slows down employees,   hence added taking away perms.                                                                   \\
		\hline
		Limited access from WebX.                                          & 1x New ICS software feature.\newline 5x Taking away permissions.                                                         & Limiting WebX access is mostly   about finding the features which may be dangerous and are not needed at all   times; and disabling them. Some employees will still find that not being able   to do everything slows them down. \\
		\hline
		WebX reduced to site   monitoring.                                 & Above +\newline 3x Extra employee.\newline 5x Taking away permissions.                                                   & Once “write-access” is disabled   in WebX, we need to have more employees at the site to have access to ViewX.                                                                                                                   \\
		\hline
		Access levels introduced to   ViewX.                               & 1x New ICS software feature\newline 1x New employee\newline 2x Taking away permissions.                                  & That is a new feature in ViewX   and we need a person responsible for managing access rights. Most employees   will now have a limited control.                                                                                  \\
		\hline
		Yearly updates                                                     & 2x New PC software\newline 3x Extra employee                                                                             & Updates were avoided mostly due   to workload involved with manually updating all air-gapped devices. Employees   are needed to test the updates before releasing them.                                                          \\
		\hline
		Monthly updates                                                    & Above +\newline 5x Extra employee.                                                                                       & Higher update intensity.                                                                                                                                                                                                         \\
		\hline
		Testing all updates in the test   system                           & 4x New employee\newline 10x Buying a tool\newline 10x New PC software\newline 5x New PLC infrastructure                  & A separate test system needs to   be built to a high cost.                                                                                                                                                                       \\
		\hline
		Code signing on PCs                                                & Above +\newline 20x New PC software\newline 5x New ICS software feature                                                  & We need to pay to have all our   software signed and the infrastructure to check the signatures.                                                                                                                                 \\
		\hline
		Code signing on PCs and PLCs                                       & Above +\newline 5x New PLC infrastructure                                                                                & Our PLCs do not support this.   We need to pay for locking them down to signed software.                                                                                                                                         \\
		\hline
		DES Encryption                                                     & 2x New ICS software feature                                                                                                                                      & It is assumed we need to   implement it in software at both sides of the communication.                                                                                                                                          \\
		\hline
		AES Encryption                                                     & Above +\newline 2x New PLC infrastructure                                                                                & In addition to the software, we   need to buy new hardware.                                                                                                                                                                      \\
		\hline
		2FA with a personal device                                         & 1x Buying a tool\newline 2x Extra employee\newline 1x New ICS software feature\newline 1x Taking away rights             & The on-going costs are mostly   associated with IT support having to handle key resetting securely. Possible   loss of productivity.                                                                                             \\
		\hline
		2FA with an issued key                                             & Above +\newline 5x Buying a tool.\newline 1x Extra employee.\newline 3x Taking away rights                               & Keys need to be bought.   Employees need to get them from the office, consuming their time.                                                                                                                                      \\
		\hline
		Company-provided devices used.                                     & Above +\newline 10x Buying a tool.\newline 2x taking away rights.                                                        & An assumption is made that we   need 10 laptops. An administrator is needed to lock down the devices to   access only WebX.                                                                                                      \\* \bottomrule
	\end{xltabular}
\end{landscape}


==> tables/model_data.tex <==
\begin{landscape}
	\begin{table}[ht]
	    \caption{Control groups and levels.}
		\label{tab:appendix_controls} \\
		\begin{tabularx}{\columnwidth}{ccXccc}
			ID & Control name & Level name & D.\footnotemark[1] & I.\footnotemark[2] & F.\footnotemark[3]  \\
			\hline
			\multirow{3}{*}{NSeg} & \multirow{3}{*}{Network segmentation}& ViewX and OT Active Directory removed from IT zone. & 60 & 138 & 0.5 \\
								  & & Access to OT from IT limited to WebX. & 120 & 276 & 0.2 \\
								  \hline
			\multirow{4}{*}{USB} & \multirow{4}{*}{USB devices}& Company issued and periodically formatted drives only. & 10 & 80 & 0.5 \\
								 & & Single-use CDs only recorded directly by SCADA software. & 52 & 170 & 0.2 \\
								 \hline
			\multirow{2}{*}{WebAcc} & \multirow{2}{*}{WebX access policy}& Limited access from WebX. & 45 & 210 & 0.5 \\
									& & WebX reduced to site monitoring. & 65 & 410 & 0.1 \\
									\hline
			\multirow{1}{*}{ViewAcc} & \multirow{1}{*}{ViewX access policy}& Access levels introduced & 49 & 170 & 0.5 \\
			\hline
			\multirow{2}{*}{Upd} & \multirow{2}{*}{Update site machines}& Yearly updates & 19 & 16 & 0.7 \\
								 & & Monthly updates & 44 & 16 & 0.5 \\
								 \hline
			\multirow{3}{*}{Sign} & \multirow{3}{*}{Code signing and testing}& Code testing & 550 & 160 & 0.5 \\
								  & & Code signing on PCs & 790 & 370 & 0.2 \\
								  & & Code signing on PCs and PLCs & 1290 & 370 & 0.1 \\
								  \hline
			\multirow{2}{*}{Wifi} & \multirow{2}{*}{Wireless security}& DES encryption & 80 & 20 & 0.5 \\
								  & & AES encryption & 280 & 20 & 0.05 \\
								  \hline
			\multirow{2}{*}{IT} & \multirow{2}{*}{IT network protection}& Firewall, antivirus and patch manager installed on thin clients. & 11 & 24 & 0.8 \\
			\hline
			\multirow{3}{*}{WebAuth} & \multirow{3}{*}{WebX authorisation}& 2FA with a personal device & 52 & 58 & 0.6 \\
									 & & 2FA with a physical key & 65 & 218 & 0.3 \\
									 & & Company-provided devices used & 77 & 378 & 0.1 \\
									 \hline
			\multirow{2}{*}{ViewAuth} & \multirow{2}{*}{ViewX authorisation}& 2FA with a personal device & 52 & 58 & 0.5 \\
									  & & 2FA with a physical key & 65 & 218 & 0.2 \\
									  \hline
		\end{tabularx}
		\footnotemark[1]{\footnotesize Direct cost.}
		\footnotemark[2]{\footnotesize Indirect cost.}
		\footnotemark[3]{\footnotesize Flow reduction.}

	\end{table}
\begin{table}[ht]
    \caption{Edges, default flows and applicable controls.} Numbers in brackets specify flow reductions different from specified in \autoref{tab:appendix_controls}. In this case, it is used because some edges benefit only from code testing (infection via vendor) while others benefit only from code signing (USB replication).
	\label{tab:appendix_edges} \\
	\begin{tabular}{c c p{14em} c c}
		\toprule
		Source & Target & Vulnerability & Default flow & Controls \\
		\midrule
		The Internet & Home PC or laptop & Spearphishing Attachment & 0.9 & WebAuth \\
		The Internet & Home PC or laptop & Drive-by Compromise & 0.6 & WebAuth \\
		The Internet & Corporate thin client & Spearphishing Attachment & 0.9 & IT \\
		The Internet & Corporate thin client & Drive-by Compromise & 0.6 & IT \\
		The Internet & Vendor software & Supply Chain Compromise & 0.3 &  \\
		The Internet & Site machine & Replication Through USB & 0.2 & Sign[1,0.5,0.5], USB, Upd \\
		Vendor software & Corporate thin client & Infection via vendor & 0.66 & Sign[0.5,0.5,0.5], IT \\
		Vendor software & Test system & Deployed for testing & 0.33 &  \\
		Test system & Site machine & Deployed for production & 1 & Sign[0.4,0.1,0.1] \\
		Test system & ViewX & Deployed for production & 1 & Sign \\
		Site machine & Control system & Exercise full control & 1 & ViewAcc \\
		ViewX & Control system & Exercise full control & 1 & ViewAcc \\
		WebX & Control system & Exercise limited control & 1 &  \\
		Home PC or laptop & WebX & Execution through API & 0.3 & WebAcc \\
		The Internet & Site machine & Wireless Compromise & 0.2 & Wifi \\
		Corporate thin client & OT AD & Access OT AD & 0.2 & NSeg \\
		OT AD & WebX & Valid Accounts & 0.8 & WebAcc \\
		OT AD & ViewX & Lateral movement & 0.2 & ViewAuth, NSeg \\
		Corporate thin client & ViewX & Remote File Copy & 0.3 & ViewAuth, NSeg \\
		The Internet & Home PC or laptop & Valid Accounts & 0.8 & WebAuth \\
		\bottomrule
	\end{tabular}
	
\end{table}
\end{landscape}

